Left-eigenvectors are certificates of the Orbit Problem

This paper investigates the connexion between the Kannan-Lipton Orbit Problem and the polynomial invariant generator algorithm PILA based on eigenvectors computation. Namely, we reduce the problem of generating linear and polynomial certificates of non-reachability for the Orbit Problem for linear transformations with rational coefficients to the generalized eigenvector problem. Also, we prove the existence of such certificates for any transformation with integer coefficients, which is not the case with rational coefficients.

==> props/case_0.tex <==
% \begin{Lemma} 
% \todo{Mais pour la non-atteignabilité c'est un peu l'inverse: si $v_Y$ n'est pas
% la bonne combinaison linéaire, on n'atteindra pas $Y$. Il y a donc des cas
% qu'on peut éliminer trivialement sans même considérer $A'$}
 The problem of generating non-reachability certificates for an orbit instance $\orbit(A,X,Y)$
 can be reduced to the problem of generating reachability certificates for an orbit
 instance $\orbit(A',X',Y')$ where $A'$ is invertible.
% \end{Lemma}




==> props/case_4_certif.tex <==
 
 For a given instance $\orbit(A,X,Y)$ such that $A$ is diagonalizable and all its eigenvalues have a modulus of $1$, 
 eigenvectors can be used as semialgebraic certificates iff $Y$ is not in the closure.
%  
%   
%  , and a linear irrational certificate if 
%  $Y$ belong to the closure.
%  



==> props/case_4_certif_proof.tex <==
 
Let $\orbit(A,X,Y)$ be an instance of the Orbit Problem with $A$ a 
diagonalizable matrix only admitting eigenvalues 
$\lambda$ such that $|\lambda| = 1$
% 
Let $\varphi$ an eigenvector of $A$, we denote 
$R = \{v | \exists k. A^kX = v \}$ the reachable set.
% 
\begin{Lemma}\label{lemma_case4}
 Let $(\lambda_i,\varphi_i)$ be $d$ couples of eigenvalue / left-eigenvector of a diagonalizable 
 matrix $A$ of size $d$.
 Then
 $R = \{v|\exists k, \forall 1 \geqslant i \geqslant d, \varphi_i.v = \lambda_i^k X\}$ 
 \end{Lemma}
\begin{proof}
  Let $R' = \{v|\exists k, \forall 1\geqslant i\geqslant d, \varphi_i.v =
  \lambda_i^k X\}$.
By the definitions of $R$ and $\varphi_i$, the inclusion $R \subset R'$ is
trivially true. Now take $v\in R'$.
%  
% 
 As there exist $d$ different and independent eigenvectors, $v$ is a solution of the following 
 relation: 
  $\exists k. \Phi v = (\lambda_1^kx_1,...\lambda_d^kx_d)^t$, where $\Phi$ is an 
 invertible matrix whose lines are directly defined by eigenvectors.
%  
 As $\Phi$ is invertible, there exists only one solution for each $k$.
 As $v$ is 
 one of those solutions, then $v \in R$.
 \end{proof}

% 
By lemma~\ref{lemma_case4}, for any $i$ between $1$ and $d$,
every element $v$ of $R$
verifies $|\scalprod {\varphi_i} v| = |\scalprod {\varphi_i} X|$, thus $R \subset R_\varphi = \{v : |\scalprod {\varphi_i} v| = |\scalprod {\varphi_i} X|\}$.
% 
Note that this inclusion is strict, as $X' = A^{-1}X \in R_\varphi$ but $X' \notin R$.
% 
If $Y$ does not belong to $R_\varphi$, then $(0,R_\varphi)$ is a
non reachability certificate.
%  
% If $\forall \varphi, Y\in R_\varphi$, $Y$ may still not be reachable.
% % 
% We know that $\forall \varphi A^kX = \lambda^kX$, where $\lambda = e^{i\theta_\lambda}$.
% % 
% If $Y \in R_\varphi$, then $|\varphi Y| = |\varphi X|$.
% % 
% $Y$ is then reachable iff the argument of $\varphi Y$, that we denote $\theta_Y^\varphi$,
% is reached by the rotation performed by $A$.
% 
% $\begin{array}{llll}
% \exists k. & \theta_Y^\varphi &=& arg(\varphi A^k X)\\
% \exists k. & \theta_Y^\varphi &=& \theta_X^\varphi + k.\theta_\lambda [2\pi]\\
% \exists k.k' & \theta_Y^\varphi &=& \theta_X^\varphi + k.\theta_\lambda + 2k'\pi\\
%  \end{array}
%  $
%  
% The couple $(0, \{v | \exists k\in \mathbb{N}.k'\in{\mathbb{Z}}. \theta_v^\varphi = \theta_X^\varphi + k.\theta_\lambda + 2k'\pi \})$
% is a linear irrational certificate of non reachability


==> props/eigenvalue_not_one.tex <==
Let $\orbit(A,X,Y)$ be an unsatisfiable instance of the Orbit problem
with $A\in\mathcal M_n(\mathbb{\mathcal Q})$ admitting at least one eigenvalue $\lambda \in \mathbb C$ 
such that $|\lambda| \neq 0$ and $|\lambda| \neq 1$.
% 
Then left eigenvectors of $\Psi_d (A)$ provide : 
\begin{itemize}
 \ib real linear semialgebraic certificates for $d = 1$ ($\Psi_1 (A) = A$) if there exist real eigenvalues;
 \ib real semialgebraic certificates of degree $2$ for $d = 2$ if there exist complex eigenvalues;
 \ib at least one rational certificate of degree $n$ for $d = n$ if $|det(A)| \neq 1$.
\end{itemize}



==> props/eigenvalue_not_one_proof.tex <==
We treat each case separately:
\begin{itemize}
 \ib The case where $A$ admits real eigenvalues is treated by Property~\ref{eigenvector_n};
 \ib If $A$ admits a complex eigenvalue $\lambda$, $A$ also admits its conjugate
 $\bar \lambda$ as eigenvalue.
%  
 By Property~\ref{pilat_mul_ev}, $\Psi_2(A)$ admits $\lambda.\bar\lambda$ as a real eigenvalue,
 which is treated by Property~\ref{eigenvector_n};
%  
 \ib 
    The product of all eigenvalues of a rational matrix is rational. 
%     
    As such, $\Psi_n$ necessarily admit a rational eigenvalue which implies the existence 
    of an associated rational eigenvector that can be used, according to Property~\ref{eigenvector_n}, 
    as a certificate.
    
\end{itemize}


==> props/eigenvector_n.tex <==
% \begin{Prop}
Let $A \in \mathcal M_d(\q)$ a linear transformation and $\orbit(A,X,Y)$ an instance 
of the Orbit problem with no solution.
Searching for a non-reachability certificate of an instance of the Orbit problem
when $A$ admits real eigenvalues $\lambda$ such that $|\lambda| \neq 0$ and $|\lambda|\neq 1$
can be reduced to computing the eigenvector decomposition of $A$.

~

\noindent
More precisely, if there exists $\varphi$ a $\lambda$-left-eigenvector of $A$ with $|\lambda| \neq 0$ and $|\lambda| \neq 1$,
% and $|\lambda| \neq 0$,
then there necessarily exists $N$ such that the 
couple $(N,P)$ defined as follows is a non-reachability
certificate of $\orbit(A,X,Y)$.

\begin{enumerate}
 \item If $|\scalprod \varphi X| \neq 0$ and $|\scalprod \varphi Y| = 0$, 
 then $N = 0$ and $P = \{v: \scalprod\varphi v \neq 0\}$
 
 \item If $|\scalprod \varphi X| = 0$ and $|\scalprod \varphi Y| \neq 0$, 
 then $N = 0$ and $P = \{v: \scalprod\varphi v = 0\}$.
 
 \item If $|\scalprod \varphi X| \neq 0$ and 
 $|\scalprod \varphi Y| \neq 0$, $N = max(1,\lfloor\frac{ln(|\scalprod\varphi Y|) - ln(|\scalprod{\varphi}{X}|)}{ln (|\lambda|)}\rfloor + 1)$ and
 \begin{itemize}
 \ib If $|\lambda| > 1$, then $P = \{v: |\scalprod\varphi v| \geqslant |\lambda.\scalprod \varphi Y|\}.$
 \ib If $|\lambda| < 1$, then $P = \{v: |\scalprod\varphi v| \leqslant |\lambda.\scalprod \varphi Y|\}.$
\end{itemize}

 \item
   Otherwise, if $d > 1$ there exist a transformation $B\in \mathcal M_{d-1}(\q)$ such that the problem of 
 finding a certificate for $\orbit(A,X,Y)$ can be reduced to the problem of finding a certificate
 for $\orbit(B,X,Y)$. 
 
 If $d = 1$, then $\orbit(A,X,Y)$ has a solution.
 
 \end{enumerate}

\noindent
The certificate is semi-linear iff $\lambda \in \mathbb Q$.
% \end{Prop}


==> props/eigenvector_n_proof.tex <==
Let $\varphi$ be a left-eigenvector of $A$ associated to the eigenvalue
$\lambda$.
% 
We know that for all $v$, $\scalprod{\varphi}v = k \Rightarrow \scalprod{\varphi}{Av} = \lambda.k$.
% 
Let $U_n = |\scalprod{\varphi}{A^nX}|$ be the $n$-th reachable state from $X$.
% 
If $|\lambda| < 1$ (resp. $|\lambda| > 1$), then $(U_n)$ is strictly decreasing (resp. strictly increasing).
% 
% Assuming $k_Y \neq 0$ and $U_0 \neq 0$, then there necessarily exist a $N$ such that 
% if 
\begin{enumerate}
 \item Let $k_v = |\scalprod{\varphi}{v}|$.
If $k_X \neq 0$ and $k_Y = 0$, then the sequence $(U_n)$ never reaches
$k_Y$, as for all $n$, $U_n \neq 0$.
% 
In other words, $|U_n| > 0$ for all $n \in \n$. 
% 
Then it is clear that $P = \{X: |\scalprod \varphi X| \neq 0\}$ is a valid certificate set
of index $N = 0$.
% 
\item
Similarly, if $k_X = 0$ and $k_Y \neq 0$, then $P = \{X: |\scalprod \varphi X| = 0\}$ and
$N = 0$.
% 


\item
Assume now that $k_X \neq 0$ and $k_Y \neq 0$.
% % 
% If $U_0 < k_Y$, $Y$ is clearly not reachable as the decreasing sequence $(U_n)$
% can never take the value $k_Y$.
% 
If $k_X < k_Y$ and $|\lambda| < 1$ (respectively $k_X > k_Y$ and $|\lambda| > 1$), then 
$(1,\{v: |\scalprod \varphi v| \leqslant |\lambda|.k_Y\})$ is a valid certificate set (respectively
$(1,\{v: |\scalprod \varphi v| \geqslant |\lambda|.k_Y\})$).
% 
Otherwise, let us assume $|\lambda| < 1$ and $k_x\geq k_y$.
% 
$U_n$ is strictly decreasing, so there exist a $N$ such that $U_N \geqslant k_Y$ and
$U_{N+1} < k_Y$.
% 
This implies that $Y$ can only be reachable after a finite number of iterations $N$.
% 
We also have that $U_{N+1} \geqslant |\lambda|.k_Y$ and $U_{N+2} < |\lambda|.k_Y$.
% 
If for all $n < N+1$, $Y \neq A^nX$, we can
% 
define $P = \{v: |\scalprod \varphi v| < |\lambda|.k_Y \}$, and obtain $Y \notin P$ 
and $\{A^{N+1+n}X | n\in\mathbb N\} \subset P$.
%
% 
Therefore, the couple $(N+1,P)$ is a non-reachability certificate of $\orbit(A,X,Y)$.
% 
A similar proof for $|\lambda|>1$ is valid as the sequence $U_n$ is now strictly increasing and
the couple $(N,\{|\scalprod \varphi X| \geqslant |\lambda|.k_Y \})$ is the corresponding certificate.

We will now study the exact value of $N$. 
% 
If $Y$ is reachable, then there exists a unique value of $N$ such that
$|\lambda|^N|\scalprod\varphi X| = k_Y$.
% 
This value is precisely $\frac{ln(|\scalprod\varphi Y|) - ln(|\scalprod{\varphi}{X}|)}{ln (|\lambda|)}$.
% 
If for every value of $n \leqslant N$, $Y$ is not reached and as $Y$ noes not 
belong to the certificate set $P$, the couple $(max(0,\lfloor N\rfloor), P)$ is
a non-reachability certificate.
% \todo{les items font un peu bizarre dans cette preuve}

\item
Assume $k_X = k_Y = 0$. 
% 
In this case for every $n$, $\scalprod \varphi {A^nX} = 0$, thus the
linear combination of variables $\varphi.X$ is always equal to $0$.
% 
There exists a base $\mathcal B$ of the transformation in
which there exists a variable $v$ which remains null for every iteration
of the transformation.
% 
In other words, there exist $A',Q$ such that $A' = Q.A.Q^{-1}$. 
% 

Assume $d > 1$ and let $B'=A_{|_{V\backslash v}}'$ and $Q' = Q_{|_{V\backslash v}}$ the transformations 
restricted to all variables but $v$ (by removing both the associated line and column).
% 
Finding a certificate for $A$ is reduced to finding a certificate for $B = Q'^{-1}B'Q'$.

If $d = 1$ and there exist a linear combination $\varphi$ of $X$ such that 
$\scalprod \varphi X = 0$, then $X = 0$.
% 
Similarly, $Y = 0$.

\end{enumerate}

Concerning the linearity of the certificate,
% 
if $\lambda \in \mathbb Q$, then every coefficient of $\varphi$ also
belongs to $\mathbb Q$.
Indeed $A$ has rational coefficients, so does $\varphi A = \lambda.\varphi$.
Similarly, if $\varphi$ has rational coefficients, $\varphi.A = \lambda.\varphi$ also does.

In the case of $k_X \neq 0$ and $k_Y  \neq 0$, we also have to get rid of the 
absolute value around $\scalprod \varphi v$ in the definition of the certificate set.
% 
If $|\lambda| > 1$, the certificate set
$\{v: (\scalprod \varphi v \geqslant |\lambda \scalprod \varphi Y|) \wedge (\scalprod \varphi v \leqslant -|\scalprod \varphi Y|)\}$
is semilinear.
% 
A similar set can be found for $|\lambda| < 1$.
% 
% \ib
%  If $U_0 = 0$, then by definition, $\forall n, U_n = 0$.
%  If $k_Y \neq 0$, then  $(0,\{v. |\scalprod\varphi v| = 0\})$ is a valid certificate.
% 
% % \ib 


==> props/eigenvector_poly.tex <==
 
% \begin{Prop}
 Let $A$ a linear transformation and $\{e_i\}_{i < N}$
 $N$ linked $1$-left eigenvectors (i.e. $e_0A=e_0$ and for $0<i<N$,
 $e_iA = e_i + e_{i-1}$).
 Then for all $i < N$, 
%  
 $\scalprod{e_iA^k}{X} = P_i(k,X)$, where $P_i(k,X)$ is a polynomial 
 of degree $i$ in the variable $k$ and $1$ in each variable of $X$.
%  

% \end{Prop} 


==> props/eigenvector_poly_proof.tex <==
Let $\{e_i\}_{i<N}$ a family of $N$ linked 1-left eigenvectors.
% 
We can compute $P_i(k,X)$ by induction on $i$.
% 
For $i = 0$, $e_0$ verifies $e_0A^k = e_0 = {k \choose i} e_{N-i-1} $.
% 
Assume now $e_{i}A^k= P_{i}(k)$ are vectors of polynomials of degree at 
most $i$. Then, we have
% 
$e_{i+1}.A^{k+1} = (e_{i+1} + e_i).A^k = e_{i+1}A^k + P_i(k)$
%$
%\begin{array}{lll}
% e_{i+1}.A^{k+1} &=& (e_{i+1} + e_i).A^k\\
% &=& e_{i+1}A^k + P_i(k)
%\end{array}
%$
Now, let $U_{k+1} = U_k + P_i(k)$.
% 
Then $U_k = U_0 + \sum\limits_{l=0}^k P_i(l)$ is a vector of polynomials of degree at most $i + 1$.


==> props/gen_eigen_certif.tex <==
Let $\orbit(A,X,Y)$ be a non satisfiable instance of the Orbit Problem
such that for all eigenvalue $\lambda$ of $A$, $|\lambda| = 1$
and $A$ is not diagonalisable.
% 
Then there exist a family of $1$-left-eigenvectors $\mathcal F = \{e_0,...,e_n\}$ 
of $\Psi_2(A)$ such that for all $1 \leqslant i \leqslant n$, 
$Q_i(n) = \scalprod {e_i} {\Psi_2(A)^n\Psi_2(X)}$ is a polynomial and $(N,P)$ is a 
non reachability certificate with:

\begin{itemize}
 \ib $N = \lfloor max(\{0\} 
%  \cup \{ x \in \mathbb R. Q'(x) = 0\} 
 \cup \{x \in \mathbb R. Q(x) = \scalprod {e_i} {\Psi_2(A^x)\Psi_2(Y)}\}) \rfloor$
 \ib $P = \{v : |\scalprod {e_i} {\Psi_2(A)^n\Psi_2(v)}| \geqslant |Q(N)|  \}$
\end{itemize}


==> props/gen_eigen_certif_proof.tex <==
Let $\orbit(A,X,Y)$ be an instance of the Orbit Problem.
% 
We will reduce the problem to the case where $A$ has positive rational eigenvalues, i.e. $\lambda = 1$ 
and $A$ admits a family $\mathcal F$ of left-eigenvectors of size $|\mathcal F| > 1$ .
% 
In this case, by Property~\ref{eigenvector_poly} we know that there exists a linear
combination of variables $v$ following a polynomial evolution described by 
$Q$ such that $deg(Q) > 0$.
% 
As $Q$ eventually diverges, there exists a $N$ such that for all $N' > N$, 
$|v(A^{N'}X)| > |v(Y)|$.
% 
This $N$ is the maximum between $0$ and the highest value of $x$ such that $Q(x) = v(Y)$
as, for any higher value of $x$, $|Q(x)| > |v(Y)|$.
% 
Also, the set $\{v . |\scalprod {e_i} {\Psi_2(A)^n\Psi_2(v)}| \geqslant |Q(N)|\}$ contains 
all reachable configurations but does not contain $Y$, thus $(N,P)$ is a valid certificate.

In the general case where $\lambda \in \mathbb C$, we will use Property~\ref{pilat_mul_ev} to show that
if there exist complex eigenvalues $\lambda$ such that $|\lambda| = 1$, of
multiplicity $m > 1$ with $m  \neq dim(ker(A - \lambda Id))$, then $\Psi_2(A)$ admits $1$ or $-1$ 
as an eigenvalue and its multiplicity $m' >1 \neq dim(ker(\Psi_2(A) - \lambda Id))$.
% 
This implies directly the existence of generalized eigenvector, thus of a family of left-eigenvectors of size 
strictly higher than $1$.
% 
To this purpose, we refer to basic properties of $\Psi_d$: 
% 

  \begin{Lemma}~\label{prop:intermediate_lemma}
    \begin{enumerate}
      \item  $\Psi_k(A.B) = \Psi_k(A).\Psi_k(B)$ 
      \item  $\Psi_k(A^{-1}) = \Psi_k(A)^{-1}$ 
      
    \end{enumerate}
  \end{Lemma}
  \begin{proof}    
    \begin{enumerate}
      \item $\Psi_k(A).\Psi_k(B)p(X)= \Psi_k(A).p(B.X) = p(A.B.X) = \Psi_k(A.B)p(X)$
      \item $\Psi_k(A^{-1}).\Psi_k(A) . p(X) = p(A.A^{-1}X) = p(X)$
      so $\Psi_k(A^{-1}).\Psi_k(A) = Id$.
    \end{enumerate}
  \end{proof}

Let $J$ the Jordan normal form of $A$, i.e. there exists $P$ such that $A = P^{-1}JP$.
%   
We have that
      $J =\left(
	  \begin{array}{cccc}
	    J_1 & 0 &... &0\\
	    0 & \ddots &  \ddots & \vdots\\
	    \vdots & \ddots & \ddots & 0\\
	    0 & ... & 0 & J_k
	    \end{array}\right) $,
% 	    
	    and
% 	    
	    $J_k = \left(
	  \begin{array}{cccc}
	    \lambda_k & 1 &  ... &0\\
	    0 & \ddots  & \ddots &\vdots\\
	    \vdots & \ddots & \ddots & 1\\
	    0 & ... & 0 & \lambda_k
	    \end{array}\right) $
% 



  From Lemma~\ref{prop:intermediate_lemma}, it is easy to prove that 
  $\Psi_d(A) = \Psi_d(P)^{-1}\Psi_d(A)\Psi_d(P)$.
%   
  As $\Psi_d(A)$ and $\Psi_d(J)$ are similar, they have the same eigenvalues.
%   
%     
%   \begin{Def}
%    Let $f$ a linear application. We define a 
%    \emph{dependency order} $\prec_f$ on $Var$ a total order such that 
%    for all $x \in Var$, $f(X)$ restricted to $x$
%    depends only on a linear combination of variables $V$ for which 
%    $\forall y \in V, y \preceq_f x$. We also say that $f$ respects $\prec_f$.
%   \end{Def}
% 
%   Given the order of variables $\prec_J$, the lexicographic order of monomials  $\prec_{\Psi_2(J)}$ of variables with 
%   respect to $\prec_J$ makes $\Psi_2(J)$ upper triangular.
% %   
%   Indeed, let us take $x_J$ and $y_J$ two variables. Their images are
%  respectively
%  $\lambda_x.x_J + v_x$ and $\lambda_y.y_J + v_y$ where $v_x$ and $v_y$ are variables verifying 
%   $v_x \prec_J x_J$ and  $v_y \prec_J y_J$.
% %   
%   Then the image of the monomial $x_J.y_J$ will be $\lambda_x.\lambda_y.x_J.y_J + \lambda_x.y_J.v_x + \lambda_y.x_J.v_y + v_x.v_y$, where
%   $y_J.v_x \prec_{\Psi_2(J)}x_J.y_J$, $x_J.v_y\prec_{\Psi_2(J)}x_J.y_J$ and $v_x.v_y\prec_{\Psi_2(J)}x_J.y_J$
% %   
% 
%  $\Psi_2(J)$ is then upper triangular and has on its diagonal every product of eigenvalues. 
%  
 We know that there exist $v_1,v_2,v_3$ in the base of $J$ 
 such that 
 \begin{itemize}
  \item $v_1' = \lambda.v_1 + v_2$
  \item $v_2' = \lambda.v_2$
  \item $v_3' = \bar\lambda.v_3$
 \end{itemize}
where $v_i'$ is the new value of $v_i$ in the base of $J$.
% 
 Then the image of $v_1v_3$ (denoted $(v_1v_3)'$) with respect to
 $\Psi_2(J)$ is $v_1v_3 + \bar\lambda.v_2.v_3$.
% 
Also, we know that $(v_2v_3)' = v_2 v_3$.
% 
 Let $\varphi$ such that $\varphi.\Psi_2(J).V = v_1v_3$.
 
%  
$
 \begin{array}{lll}
  
 \varphi.(\Psi_2(J) - Id) V& = &v_1v_3 \bar\lambda.v_2v_3 - v_1v_3\\
 & = & \bar\lambda.v_2v_3\\
 \varphi.(\Psi_2(J) - Id)^2 V& = &\bar\lambda.v_2v_3 - \bar\lambda.v_2v_3\\
 \varphi.(\Psi_2(J) - Id)^2 V& = & 0
 
 \end{array}$
 
 As this is true for any $V$, then $\varphi .(\Psi_2(J) - Id) \neq 0$ and $\varphi.(\Psi_2(J) - Id)^2 = 0$.
%  
In conclusion, $\varphi$ is a generalized eigenvector of $\Psi_2(J)$, thus $\Psi_2(A)$ 
also admits a generalized eigenvector.

% %  
%  If $A$ admits an eigenvalue $\lambda \in \c$ such that $|\lambda| = 1$, it also admits as eigenvalue $\bar \lambda$.
% Since $\lambda\bar\lambda = 1$, $1$ appears on the diagonal of $\Psi_2(J)$.


==> props/integ_op_solv.tex <==
Any non-reachable instance of the Orbit problem $\orbit(A,X,Y)$ where 
$A \in \mathcal{M}_n(\mathbb{Z})$ admit a closed semi-algebraic invariant.


==> props/integ_op_solv_proof.tex <==
We already treated the case where the matrix has an eigenvalue whose modulus 
is different from $1$ (Property~\ref{eigenvector_n}) and the case where the matrix 
is not diagonalizable (Property~\ref{eigenvector_poly}).
% 
We are left with the hypothesis of the Property~\ref{kronecker}.
% 

Let $A$ be a transformation such that all its eigenvalue are either $0$
or roots of unity.
% 
$A$ represents a finite-monoïd transformation, i.e. its reachable set of space
is \emph{finite}. 
% 
More precisely, there exist $N,p$ such that $\forall n > N, A^{n+p} = A^n$
% 
Let $P = \{A^NX,A^{N+1}X,...,A^{N+p-1}X\}$. 
% 
If $Y$ is not reachable, then the couple $(P,N)$ is a non-reachability certificate.

The closure of such a certificate comes from the same eigenvalue argument.
% 
The only case we had a non-closed certificate comes from Property~\ref{eigenvector_n}
when $|\lambda|\neq 0$, $|\lambda|\neq 1$, $|\scalprod \varphi X| \neq 0$ and 
$|\scalprod \varphi Y\ \neq 1$.
% 
As we also have $|\lambda|\geqslant 1$ for integer matrices, the certificate set 
$\{v: |\scalprod \varphi v| \geqslant |\scalprod \varphi X| \}$ is a valid closed 
certificate set.


==> props/kronecker.tex <==
% \begin{Prop}
  Let $A \in \mathcal{M}_n(\z)$. 
  If all its eigenvalue $\lambda$ have a modulus inferior or 
  equal to $1$, then there exists $n > 1$ such that $\lambda^n = \lambda$.
% \end{Prop}


==> props/kronecker_proof.tex <==
Let $A \in \mathcal{M}(\z)$ such that for all eigenvalue $\lambda$,
$|\lambda| \leqslant 1$.

If $\lambda = 0$, then we can conclude right away ($0^2 = 0$).

The characteristic polynomial $P\in\mathbb{Z}[X]$ of $A$ is monic, i.e. its leading coefficient is
$1$. Thus by definition, every eigenvalue is an algebraic integer.
% 
We will use the Kronecker theorem~\cite{schinzel1965refinement}, stating that if a non null algebraic integer 
$\alpha$ has all its rational conjugates (i.e. roots of its rational minimal polynomial) 
admitting a modulus inferior or equal to $1$, then $\alpha$ is a root of unity.

Each eigenvalue $\lambda$ admits a minimal rational polynomial $Q$. 
% 
We can show that $Q$ necessarily divides $P$ by performing an euclidian
division : there exist $D,R \in \mathbb{Q}[X]$ such that $P(X) = Q(X)D(X) + R(X)$,
with the degree of $R$ strictly inferior to $Q$.
% 
We know that $P(\lambda) = 0$ and $Q(\lambda) = 0$, thus $R(\lambda) = 0$.
% 
If $R \neq 0$, then $R$ is the minimal polynomial of $\lambda$ as its degree is inferior 
to the degree of $Q$, which is absurd by hypothesis.
% 
Thus, the set of rational conjuguates of $\lambda$ are roots of $P$,
by hypothesis of modulus inferior or equal to $1$.
% 
By the Kronecker theorem, $\lambda$ is a root of unity, i.e. $\exists n > 1. \lambda^n = \lambda$.
 


==> props/pilat_mul_ev.tex <==

  Let $A\in\mathcal{M}_d(\mathbb{Q}),\Lambda(M)$ the eigenvalue set of a
  matrix $M$ and $k$ an integer.
%   
  Then for any product $p$ of $k$ or less elements of $\Lambda(A), p \in \Lambda(\Psi_k(A))$
  where $\Psi_k(A)$ is the elevation of $A$ to the degree $k$.



==> results.tex <==
 

